Mitigating Covariate Shift in Imitation Learning via Offline Data Without Great Coverage

This paper studies offline Imitation Learning (IL) where an agent learns to imitate an expert demonstrator without additional online environment interactions. Instead, the learner is presented with a static offline dataset of state-action-next state transition triples from a potentially less proficient behavior policy. We introduce Model-based IL from Offline data (MILO): an algorithmic framework that utilizes the static dataset to solve the offline IL problem efficiently both in theory and in practice. In theory, even if the behavior policy is highly sub-optimal compared to the expert, we show that as long as the data from the behavior policy provides sufficient coverage on the expert state-action traces (and with no necessity for a global coverage over the entire state-action space), MILO can provably combat the covariate shift issue in IL. Complementing our theory results, we also demonstrate that a practical implementation of our approach mitigates covariate shift on benchmark MuJoCo continuous control tasks. We demonstrate that with behavior policies whose performances are less than half of that of the expert, MILO still successfully imitates with an extremely low number of expert state-action pairs while traditional offline IL method such as behavior cloning (BC) fails completely. Source code is provided at https://github.com/jdchang1/milo.

==> docs/check_list.tex <==


\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
   \answerYes{} See \pref{sec:intro}
  \item Did you describe the limitations of your work?
\answerYes{}  See \pref{sec:analysis}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See \pref{sec:conclusion} for a discussion}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{We have read through the ethical guidelines.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
   \answerYes{}See \pref{sec:analysis}
	\item Did you include complete proofs of all theoretical results?
   \answerYes{} See \pref{sec:analysis}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Experimental details and exact hyperparameters are reported in the supplemental material. Code and data will be released along with the camera ready version with a URL to the github repository.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{All details are enumerated and documented in the supplemental material.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{All plots and tables report error bars of the average across five random seeds.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{We use small neural networks and do not work with image inputs thus did not require GPU acceleration or specialized hardware. Each of our experiments were run on 2 cpu cores and 8GB of ram.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See \pref{sec:experiments} where we cite the creators of the assets.}
  \item Did you mention the license of the assets?
    \answerNo{For OpenAI Gym, we use their opensource software and we payed for the proprietary MuJoCo license.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
  \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
\answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
   \answerNA{}
\end{enumerate}

\end{enumerate}


==> notation.tex <==
\newcommand{\brank}{R_B} \newcommand{\mrank}{R_M}
\newcommand{\olive}{\textsc{Olive}}

